Safe to Resume? Breaking Execution Continuity of Agent Execution via Rollback

AI agents are moving toward persistent, stateful execution across various applications, accumulating execution state and external effects that are costly to reconstruct after failures. Checkpoint and rollback (C/R) are becoming essential for recovery, yet their security implications remain largely unexplored. Correct rollback does not imply secure recovery: a faithfully restored checkpoint may resume an execution whose states, assumptions, and external effects never coexisted in any valid history. In this paper, we present the first systematic security study of checkpoint and rollback in existing agent systems. By examining representative agent C/R systems, we characterize the design space of existing C/R mechanisms and develop a general execution model that captures their recovery boundaries and state dependencies. From this model, we identify five fundamental failure modes spanning incomplete or inconsistent internal state, stale external dependencies, nondeterministic replay, and unrecorded external effects. We further demonstrate their security impact through three end-to-end attacks on Hermes, Cline, and LangGraph, enabling malware-verification bypass, unauthorized mail forwarding, and double payment. To systematically study these failures in practice, we develop a multi-agent analysis pipeline that reconstructs execution semantics, identifies violations of the five failure conditions, and validates them through actual rollback. Across five representative frameworks, our evaluation shows that these failures recur across heterogeneous C/R designs and stem from a common gap between the state restored by a checkpoint and the dependencies required for secure continuation.

==> framework.tex <==

\subsection{Detection Framework}
\label{sec:framework}

\subsection{Overview}
\label{sec:analysis-overview}

Our framework identifies security failures in a given agent task and checkpointing framework that may be exploitable by an adversary. 
It operates in four stages. First, \emph{trace collection} records the complete task execution, including checkpoint contents, framework state, model and tool interactions, state changes, and interactions with the outside world. 
Second, a \emph{semantic analyzer} converts the trace into structured event facts, including each event's input dependencies, operation, outputs or effects, ordering relations, and nondeterministic behavior. 
Third, five fixed checkers analyze these event facts to identify SF1--SF5. 
Finally, a \emph{validator} reconstructs the relevant recovery execution and checks whether each reported failure can be reproduced.
We note that the framework is designed for failure detection rather than security certification, because the trace captures only the states and interactions observed during execution, rather than the complete system state.

\subsection{Concrete Design}
\label{sec:analysis-design}

\bheading{Trace collection.}
Given a task and an agent framework, we execute the task and collect the following information:

\begin{packeditemize}
    \item \textit{Execution trace.} The sequence of model calls, framework operations, state changes, and interactions with internal and external components during task execution.
    
    \item \textit{Checkpoint state.} The creation point and contents of each checkpoint produced during execution, including the framework and system states captured by the checkpoint.
    
    \item \textit{Tool interactions.} The concrete inputs and outputs of each tool invocation, including local tools or external services.
\end{packeditemize}

\bheading{Semantic event reconstruction.}
We use an LLM-based analysis agent to reconstruct the collected trace into a structured event trace. We represent each event \(e_i\) as
\[
e_i=\langle \mathsf{op}_i,\mathsf{In}_i,\mathsf{Out}_i,\mathsf{ND}_i\rangle,
\]
where \(\mathsf{op}_i\) describes the performed operation, \(\mathsf{In}_i\) contains the versioned internal or external states on which the event depends, \(\mathsf{Out}_i\) contains the versioned states produced or modified by the event, and \(\mathsf{ND}_i\) records whether the event involves nondeterminism. We further record \(e_i \prec e_j\) when \(e_i\) causally precedes \(e_j\). The resulting structured trace captures the event-level state flow and causal order used by all subsequent checkers.




\bheading{Security-failure checking.}
Given the structured event trace and checkpoint contents, we apply
five fixed rules to identify candidate failures. The checker operates
only on the original execution; whether a candidate manifests under
recovery is determined by the validator.

\begin{packeditemize}
    \item \textit{SF1.}
    For each event $e_i$ after checkpoint $C$, we examine each
    internal state in $\mathsf{In}_i$.
    We report a candidate when the required state version was
    established before $C$, is not reproduced before $e_i$, and is
    not covered by $C$.

    \item \textit{SF2.}
    For each state in $C$, we trace through $\mathsf{In}$,
    $\mathsf{Out}$, and $\prec$ to determine the state versions
    causally required to produce it.
    We report a candidate when $C$ contains a produced state together
    with an incompatible version of another captured internal state
    required along its causal path.

    \item \textit{SF3.}
    For each internal state in $C$, we trace its dependencies to
    external states appearing in $\mathsf{In}$.
    We report a candidate whenever checkpointed internal state depends
    on state outside the recovery boundary.

    \item \textit{SF4.}
    For each event $e_i$ after $C$, we examine $\mathsf{ND}_i$.
    We report a candidate when $e_i$ involves nondeterminism and its
    outcome is not preserved by $C$, such that the event will be
    re-executed after rollback.

    \item \textit{SF5.}
    For each event $e_i$ after $C$, we examine whether
    $\mathsf{op}_i$ invokes an external operation that may produce
    persistent state outside the recovery boundary.
    We report such an operation as a candidate external effect.
\end{packeditemize}

\bheading{Finding validation.}
For each candidate associated with checkpoint $C$, the validator
allows the original execution to complete, restores $C$ using the
framework's normal recovery mechanism, and re-executes the relevant
post-checkpoint execution. A candidate is reported as a finding only
when the corresponding failure condition is observed:

\begin{packeditemize}
    \item \textit{SF1.}
    We confirm SF1 when, after rollback, an uncovered internal state
    required by the re-executed event has a different version from
    that observed in the original execution, causing recovery to
    combine states from different execution points.

    \item \textit{SF2.}
    We confirm SF2 when rollback materializes the inconsistent state
    combination identified by the checker, such that one restored
    state reflects an event whose required causal predecessor is
    absent from or incompatible with another restored state.

    \item \textit{SF3.}
    We confirm SF3 when the external state on which the checkpoint
    depends has changed after checkpoint creation, and re-execution
    under this changed state produces a different transition or
    execution path from the original execution.

    \item \textit{SF4.}
    We restore the same checkpoint and re-execute the relevant
    nondeterministic operation multiple times.
    We confirm SF4 when these executions produce different outputs,
    state transitions, or downstream execution paths.

    \item \textit{SF5.}
    We confirm SF5 when an external effect produced during the
    original execution remains after rollback, while the agent is
    restored to a state before that operation, and re-execution can
    produce the external effect again.
\end{packeditemize}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{image/systemdetector.pdf}
    \caption{Detection framework overview.}
    \label{fig:detection_framework_overview}
\end{figure}



% \bheading{Finding validation.}
% For each reported finding, the validator reconstructs the corresponding recovery scenario, restores the implicated checkpoint, and re-executes the relevant events.
% It then checks whether the predicted failure condition is reproduced. The recovery procedure can be generated by an agent and completed or verified by a human expert.

